SLowRL: Safe Low-Rank Adaptation Reinforcement Learning for Locomotion

Sim-to-real transfer of locomotion policies often leads to performance degradation due to the inevitable sim-to-real gap. Naively fine-tuning these policies directly on hardware is problematic, as it poses risks of mechanical failure and suffers from high sample inefficiency. In this paper, we address the challenge of safely and efficiently fine-tuning reinforcement learning (RL) policies for dynamic locomotion tasks. Specifically, we focus on fine-tuning policies learned in simulation directly on hardware, while explicitly enforcing safety constraints. In doing so, we introduce SLowRL, a framework that combines Low-Rank Adaptation (LoRA) with training-time safety enforcement via a recovery policy. We evaluate our method both in simulation and on a real Unitree Go2 quadruped robot for jump and trot tasks. Experimental results show that our method achieves a $46.5\%$ reduction in fine-tuning time and near-zero safety violations compared to standard proximal policy optimization (PPO) baselines. Notably, we find that a rank-1 adaptation alone is sufficient to recover pre-trained performance in the real world, while maintaining stable and safe real-world fine-tuning. These results demonstrate the practicality of safe, efficient fine-tuning for dynamic real-world robotic applications.

==> graph.tex <==

\usetikzlibrary{shapes, arrows.meta, positioning, calc, fit, backgrounds}

\begin{tikzpicture}[
    node distance=0.8cm and 1cm,
    font=\sffamily\footnotesize,
    >={Latex[width=1.5mm,length=1.5mm]},
    % --- Styles ---
    frozen/.style={
        rectangle, draw=blue!60!black, fill=blue!10, dashed, thick, 
        align=center, minimum height=0.7cm, minimum width=2.0cm, rounded corners=2pt
    },
    trainable/.style={
        rectangle, draw=green!60!black, fill=green!10, thick, 
        align=center, minimum height=0.7cm, minimum width=2.0cm, rounded corners=2pt
    },
    activation/.style={
        rectangle, draw=gray!60, fill=gray!5, thick, 
        align=center, minimum size=0.5cm, rounded corners=2pt
    },
    noise/.style={
        rectangle, draw=orange!60!black, fill=yellow!10, thick, 
        align=center, minimum height=0.8cm, minimum width=2.5cm, rounded corners=2pt
    },
    sum/.style={
        circle, draw, fill=white, inner sep=0pt, minimum size=5mm, thick
    },
    layerbox/.style={
        draw=black!60, dashed, thick, inner sep=8pt, rounded corners=5pt, fill=white, fill opacity=0.4
    }
]

    % ================= MAIN INPUT (TOP) =================
    \node [font=\large\bfseries, align=center, draw, thick, rounded corners, inner sep=10pt, fill=white] (Obs) at (0,0) {Observation\\$s_0$};


    % =========================================================
    %           LEFT TRACK: CRITIC (VALUE)
    % =========================================================
    \begin{scope}[xshift=-5.0cm, yshift=-1.5cm]
        \node [font=\large\bfseries] (TitleC) at (0, 0.7) {Critic Network (Value $V$)};
        \coordinate (CriticStart) at (0,0);
        
        % Connect Obs to Critic Start
        \draw [->, thick, rounded corners] (Obs.south) -- ++(0,-0.4) -| (CriticStart);

        % --- LAYER 1 (Critic) ---
        \node [frozen, below left=0.6cm and 0.1cm of CriticStart] (w1C) {$W^C_1 s_0 + b^C_1$};
        \node [trainable, below right=0.6cm and 0.1cm of CriticStart] (lora1C) {$\frac{\alpha}{r} B^C_1 A^C_1 s_0$};
        % \node [sum, below=2.0cm of CriticStart] (sum1C) {+};

        \draw [->] (CriticStart) -- ++(0,-0.4) -| (w1C.north);
        \draw [->] (CriticStart) -- ++(0,-0.4) -| (lora1C.north);
        \node [activation, below right=0.1cm and -0.2cm of w1C] (act1C) {ELU};
        \draw [->] (w1C.south) |- (act1C.west);
        \draw [->] (lora1C.south) |- (act1C.east);
        
        % FIX: Removed background scope so it sits on top of the main background
        \node [layerbox, inner ysep=15pt, fit=(w1C) (lora1C) (w1C), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer 1}] (L1BoxC) {};

        % Activation 1
        % \node [activation, below=0.4cm of w1C] (act1C) {ELU};
        % \draw [->] (sum1C) -- (act1C);

        % --- LAYER 2 (Critic) ---
        \coordinate [below=0.4cm of act1C] (CriticL2Start);
        
        \node [frozen, below left=0.6cm and 0.1cm of CriticL2Start] (w2C) {$W^C_2 s^C_1 + b^C_2$};
        \node [trainable, below right=0.6cm and 0.1cm of CriticL2Start] (lora2C) {$\frac{\alpha}{r} B^C_2 A^C_2 s^C_1$};
        % \node [sum, below=2.0cm of CriticL2Start] (sum2C) {+};

        % \draw [->] (act1C) -- (CriticL2Start);
        \draw [->] (act1C) -- node[right, font=\scriptsize, xshift=2pt] {$s^C_1$} (CriticL2Start);
        \draw [->] (CriticL2Start) -- ++(0,-0.3) -| (w2C.north);
        \draw [->] (CriticL2Start) -- ++(0,-0.3) -| (lora2C.north);
        
        % FIX: Removed background scope
        % \node [layerbox, fit=(w2C) (lora2C) (sum2C), label={[gray]right:Layer 2}] (L2BoxC) {};
        \node [layerbox, inner ysep=15pt, fit=(w2C) (lora2C) (w2C), label={[gray,  yshift=-1.1cm , xshift=-1.2cm]right:Layer 2}] (L2BoxC) {};

        % Activation 2
        \node [activation, below right =0.1cm and -0.2cm of w2C] (act2C) {ELU};
        \draw [->] (w2C.south) |- (act2C.west);
        \draw [->] (lora2C.south) |- (act2C.east);
        % \draw [->] (sum2C) -- (act2C);

        % --- Dots ---
        \node [below=-0.30cm of act2C, font=\Large] (dotsC) {$\vdots$};
        % \draw [->] (act2C) -- (dotsC);

        % --- LAYER N (Critic) ---
        \coordinate [below=0.2cm of dotsC] (CriticMid);
        \node [frozen, below left=0.6cm and 0.1cm of CriticMid] (wNC) {$W^C_N s^C_{N-1} + b^C_N$};
        \node [trainable, below right=0.6cm and 0.1cm of CriticMid] (loraNC) {$\frac{\alpha}{r} B^C_N A^C_N s^C_{N-1}$};
        % \node [sum, below=2.0cm of CriticMid] (sumNC) {+};

        \draw [->] (dotsC) -- node[right, font=\scriptsize] {$s^C_{N-1}$} (CriticMid);
        \draw [->] (CriticMid) -- ++(0,-0.3) -| (wNC.north);
        \draw [->] (CriticMid) -- ++(0,-0.3) -| (loraNC.north);

        % FIX: Removed background scope
        \node [layerbox, inner ysep=15pt, fit=(wNC) (loraNC) (wNC), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer N}] (LNBoxC) {};

        % --- Final Critic Output ---
        \node [activation, below right=0.1cm and -0.2cm of wNC] (actNC) {ELU};
        % \draw [->] (wNC) -- (actNC);
        \draw [->] (wNC.south) |- (actNC.west);
        \draw [->] (loraNC.south) |- (actNC.east);

        \node [below=0.3cm of actNC, align=center, font=\bfseries, draw, thick, rounded corners, inner sep=6pt, fill=white] (outputC) {Value $V(s)$};
        \draw [->, thick] (actNC) -- (outputC);

        % Background Critic (Keeps background scope to stay behind)
        \begin{scope}[on background layer]
            \node [draw=red!30, fill=red!5, fit=(TitleC) (L1BoxC) (L2BoxC) (LNBoxC) (outputC), rounded corners=10pt, inner sep=10pt] {};
        \end{scope}
    \end{scope}


    % =========================================================
    %           RIGHT TRACK: ACTOR (POLICY)
    % =========================================================
    \begin{scope}[xshift=5.0cm, yshift=-1.5cm]
        \node [font=\large\bfseries] (TitleA) at (0, 0.7) {Actor Network (Policy $\pi$)};
        \coordinate (ActorStart) at (0,0);
        
        % Connect Obs to Actor Start
        \draw [->, thick, rounded corners] (Obs.south) -- ++(0,-0.4) -| (ActorStart);

        % --- LAYER 1 (Actor) ---
        \node [frozen, below left=0.6cm and 0.1cm of ActorStart] (w1A) {$W^A_1 s_0 + b^A_1$};
        \node [trainable, below right=0.6cm and 0.1cm of ActorStart] (lora1A) {$\frac{\alpha}{r} B^A_1 A^A_1 s_0$};
        % \node [sum, below=2.0cm of ActorStart] (sum1A) {+};

        \draw [->] (ActorStart) -- ++(0,-0.3) -| (w1A.north);
        \draw [->] (ActorStart) -- ++(0,-0.3) -| (lora1A.north);
        
        % FIX: Removed background scope
        \node [layerbox, inner ysep=15pt, fit=(w1A) (lora1A) (w1A), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer 1}] (L1BoxA) {};

        % Activation 1
        \node [activation, below right=0.1cm and -0.2cm of w1A] (act1A) {ELU};
        % \draw [->] (sum1A) -- (act1A);
        \draw [->] (w1A.south) |- (act1A.west);
        \draw [->] (lora1A.south) |- (act1A.east);

        % --- LAYER 2 (Actor) ---
        \coordinate [below=0.4cm of act1A] (ActorL2Start);
        
        \node [frozen, below left=0.6cm and 0.1cm of ActorL2Start] (w2A) {$W^A_2 s^A_1 + b^A_2$};
        \node [trainable, below right=0.6cm and 0.1cm of ActorL2Start] (lora2A) {$\frac{\alpha}{r} B^A_2 A^A_2 s^A_1$};
        % \node [sum, below=2.0cm of ActorL2Start] (sum2A) {+};

        % \draw [->] (act1A) -- (ActorL2Start);
        \draw [->] (act1A) -- node[right, font=\scriptsize, xshift=2pt] {$s^A_1$} (ActorL2Start);
        \draw [->] (ActorL2Start) -- ++(0,-0.3) -| (w2A.north);
        \draw [->] (ActorL2Start) -- ++(0,-0.3) -| (lora2A.north);
        
        % FIX: Removed background scope
        \node [layerbox, inner ysep=15pt, fit=(w2A) (lora2A) (w2A), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer 2}] (L2BoxA) {};

        % Activation 2
        \node [activation, below right=0.1cm and -0.2cm of w2A] (act2A) {ELU};
        % \draw [->] (sum2A) -- (act2A);
        \draw [->] (w2A.south) |- (act2A.west);
        \draw [->] (lora2A.south) |- (act2A.east);

        % --- Dots ---
        \node [below=-0.3cm of act2A, font=\Large] (dotsA) {$\vdots$};
        % \draw [->] (act2A) -- (dotsA);

        % --- LAYER N (Actor) ---
        \coordinate [below=0.2cm of dotsA] (ActorMid);
        \node [frozen, below left=0.6cm and 0.1cm of ActorMid] (wNA) {$W^A_N s^A_{N-1} + b^A_N$};
        \node [trainable, below right=0.6cm and 0.1cm of ActorMid] (loraNA) {$\frac{\alpha}{r} B^A_N A^A_N s^A_{N-1}$};
        % \node [sum, below=2.0cm of ActorMid] (sumNA) {+};

        \draw [->] (dotsA) -- node[right, font=\scriptsize] {$s^A_{N-1}$} (ActorMid);
        \draw [->] (ActorMid) -- ++(0,-0.3) -| (wNA.north);
        \draw [->] (ActorMid) -- ++(0,-0.3) -| (loraNA.north);

        % FIX: Removed background scope
        \node [layerbox, inner ysep=15pt, fit=(wNA) (loraNA) (wNA), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer N}] (LNBoxA) {};

        % --- Final Actor Output ---
        \node [activation, below right=0.1cm and -0.2 of wNA] (actNA) {ELU};
        % \draw [->] (sumNA) -- (actNA);
        \draw [->] (wNA.south) |- (actNA.west);
        \draw [->] (loraNA.south) |- (actNA.east);

        % \node [sum, below=0.8cm of actNA] (finalSumA) {+};
        % \node [noise, right=0.5cm of finalSumA] (noise) {Trainable Noise\\(std)};
        \node [below=0.3cm of actNA, align=center, font=\bfseries, draw, thick, rounded corners, inner sep=6pt, fill=white] (outputA) {Action $a \sim \mathcal{N}(\mu, \sigma)$};

        % \draw [->] (actNA) -- (finalSumA);
        % \draw [->] (noise) -- (finalSumA);
        \draw [->, thick] (actNA) -- (outputA);

        % Background Actor (Keeps background scope to stay behind)
        \begin{scope}[on background layer]
            \node [draw=blue!30, fill=blue!5, fit=(TitleA) (L1BoxA) (L2BoxA) (LNBoxA) (outputA), rounded corners=10pt, inner sep=10pt] {};
        \end{scope}
    \end{scope}

\end{tikzpicture}

==> graph2.tex <==

\usetikzlibrary{shapes, arrows.meta, positioning, calc, fit, backgrounds}

\begin{tikzpicture}[
    node distance=0.8cm and 1cm,
    font=\sffamily\footnotesize,
    >={Latex[width=1.5mm,length=1.5mm]},
    % --- Styles ---
    frozen/.style={
        rectangle, draw=blue!60!black, fill=blue!10, dashed, thick, 
        align=center, minimum height=0.7cm, minimum width=2.0cm, rounded corners=2pt
    },
    trainable/.style={
        rectangle, draw=green!60!black, fill=green!10, thick, 
        align=center, minimum height=0.7cm, minimum width=2.0cm, rounded corners=2pt
    },
    activation/.style={
        rectangle, draw=gray!60, fill=gray!5, thick, 
        align=center, minimum size=0.5cm, rounded corners=2pt
    },
    noise/.style={
        rectangle, draw=orange!60!black, fill=yellow!10, thick, 
        align=center, minimum height=0.8cm, minimum width=2.5cm, rounded corners=2pt
    },
    sum/.style={
        circle, draw, fill=white, inner sep=0pt, minimum size=5mm, thick
    },
    layerbox/.style={
        draw=black!60, dashed, thick, inner sep=8pt, rounded corners=5pt, fill=white, fill opacity=0.4
    }
]

    % ================= MAIN INPUT (TOP) =================
    \node [font=\large\bfseries, align=center, draw, thick, rounded corners, inner sep=10pt, fill=white] (Obs) at (0,0) {Observation\\$s_0$};


    % =========================================================
    %           LEFT TRACK: CRITIC (VALUE)
    % =========================================================
    \begin{scope}[xshift=-5.0cm, yshift=-1.5cm]
        \node [font=\large\bfseries] (TitleC) at (0, 0.7) {Critic Network (Value $V$) \newline Actor Network (Policy $\pi$)};
        \coordinate (CriticStart) at (0,0);
        
        % Connect Obs to Critic Start
        \draw [->, thick, rounded corners] (Obs.south) -- ++(0,-0.4) -| (CriticStart);

        % --- LAYER 1 (Critic) ---
        \node [frozen, below left=0.6cm and 0.1cm of CriticStart] (w1C) {$W^C_1 s_0 + b^C_1$};
        \node [trainable, below right=0.6cm and 0.1cm of CriticStart] (lora1C) {$\frac{\alpha}{r} B^C_1 A^C_1 s_0$};
        % \node [sum, below=2.0cm of CriticStart] (sum1C) {+};

        \draw [->] (CriticStart) -- ++(0,-0.4) -| (w1C.north);
        \draw [->] (CriticStart) -- ++(0,-0.4) -| (lora1C.north);
        \node [activation, below right=0.1cm and -0.2cm of w1C] (act1C) {ELU};
        \draw [->] (w1C.south) |- (act1C.west);
        \draw [->] (lora1C.south) |- (act1C.east);
        
        % FIX: Removed background scope so it sits on top of the main background
        \node [layerbox, inner ysep=15pt, fit=(w1C) (lora1C) (w1C), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer 1}] (L1BoxC) {};

        % Activation 1
        % \node [activation, below=0.4cm of w1C] (act1C) {ELU};
        % \draw [->] (sum1C) -- (act1C);

        % --- LAYER 2 (Critic) ---
        \coordinate [below=0.4cm of act1C] (CriticL2Start);
        
        \node [frozen, below left=0.6cm and 0.1cm of CriticL2Start] (w2C) {$W^C_2 s^C_1 + b^C_2$};
        \node [trainable, below right=0.6cm and 0.1cm of CriticL2Start] (lora2C) {$\frac{\alpha}{r} B^C_2 A^C_2 s^C_1$};
        % \node [sum, below=2.0cm of CriticL2Start] (sum2C) {+};

        % \draw [->] (act1C) -- (CriticL2Start);
        \draw [->] (act1C) -- node[right, font=\scriptsize, xshift=2pt] {$s^C_1$} (CriticL2Start);
        \draw [->] (CriticL2Start) -- ++(0,-0.3) -| (w2C.north);
        \draw [->] (CriticL2Start) -- ++(0,-0.3) -| (lora2C.north);
        
        % FIX: Removed background scope
        % \node [layerbox, fit=(w2C) (lora2C) (sum2C), label={[gray]right:Layer 2}] (L2BoxC) {};
        \node [layerbox, inner ysep=15pt, fit=(w2C) (lora2C) (w2C), label={[gray,  yshift=-1.1cm , xshift=-1.2cm]right:Layer 2}] (L2BoxC) {};

        % Activation 2
        \node [activation, below right =0.1cm and -0.2cm of w2C] (act2C) {ELU};
        \draw [->] (w2C.south) |- (act2C.west);
        \draw [->] (lora2C.south) |- (act2C.east);
        % \draw [->] (sum2C) -- (act2C);

        % --- Dots ---
        \node [below=-0.30cm of act2C, font=\Large] (dotsC) {$\vdots$};
        % \draw [->] (act2C) -- (dotsC);

        % --- LAYER N (Critic) ---
        \coordinate [below=0.2cm of dotsC] (CriticMid);
        \node [frozen, below left=0.6cm and 0.1cm of CriticMid] (wNC) {$W^C_N s^C_{N-1} + b^C_N$};
        \node [trainable, below right=0.6cm and 0.1cm of CriticMid] (loraNC) {$\frac{\alpha}{r} B^C_N A^C_N s^C_{N-1}$};
        % \node [sum, below=2.0cm of CriticMid] (sumNC) {+};

        \draw [->] (dotsC) -- node[right, font=\scriptsize] {$s^C_{N-1}$} (CriticMid);
        \draw [->] (CriticMid) -- ++(0,-0.3) -| (wNC.north);
        \draw [->] (CriticMid) -- ++(0,-0.3) -| (loraNC.north);

        % FIX: Removed background scope
        \node [layerbox, inner ysep=15pt, fit=(wNC) (loraNC) (wNC), label={[gray, yshift=-1.1cm , xshift=-1.2cm]right:Layer N}] (LNBoxC) {};

        % --- Final Critic Output ---
        \node [activation, below right=0.1cm and -0.2cm of wNC] (actNC) {ELU};
        % \draw [->] (wNC) -- (actNC);
        \draw [->] (wNC.south) |- (actNC.west);
        \draw [->] (loraNC.south) |- (actNC.east);

        \node [below=0.3cm of actNC, align=center, font=\bfseries, draw, thick, rounded corners, inner sep=6pt, fill=white] (outputC) {Value $V(s)$};
        \draw [->, thick] (actNC) -- (outputC);

        % Background Critic (Keeps background scope to stay behind)
        \begin{scope}[on background layer]
            \node [draw=red!30, fill=red!5, fit=(TitleC) (L1BoxC) (L2BoxC) (LNBoxC) (outputC), rounded corners=10pt, inner sep=10pt] {};
        \end{scope}
    \end{scope}

\end{tikzpicture}
